A Persistent Spatial Semantic Representation for High-level Natural Language Instruction Execution

Natural language provides an accessible and expressive interface to specify long-term tasks for robotic agents. However, non-experts are likely to specify such tasks with high-level instructions, which abstract over specific robot actions through several layers of abstraction. We propose that key to bridging this gap between language and robot actions over long execution horizons are persistent representations. We propose a persistent spatial semantic representation method, and show how it enables building an agent that performs hierarchical reasoning to effectively execute long-term tasks. We evaluate our approach on the ALFRED benchmark and achieve state-of-the-art results, despite completely avoiding the commonly used step-by-step instructions.

==> task.tex <==
\section{Task}
\label{sec:task}

Given a high-level natural language instruction $\taskstr$ and an initial state of the world $\state_{0}$, the goal of the agent is to generate an execution $\traj = \langle \state_{0}, \action_{0}, \state_{1}, \action_{1}, \dots, \state_T, \action_T \rangle$, where $\action_{i} \in \allactions$ is an action taken by the agent at time $i$, $\state_{i} \in \allstates$ is the world state before taking $\action_{i}$, and $\state_{i+1} = \dynamics(\state_{i}, \action_{i})$ under environment dynamics  $\dynamics : \allstates \rightarrow \allstates$.
The world state $\state_{i}$ is defined by the current room, poses and states of all objects in the room, and pose of the agent.
The agent does not have access to the world state $\state_{i}$, but only an observation $\obs_{i} \in \allobs$.
The observation $\obs_{i} = (\image_{i}, \taskstr)$ consists of a first-person RGB camera image $\image_{i}$ and the task description $\taskstr$.
The task is considered successful if all goal-conditions corresponding to the task $\taskstr$ are true at the final state $\state_T$.
Partial success is measured as the fraction of goal-conditions that have been achieved.

